StyleDomain: Efficient and Lightweight Parameterizations of StyleGAN for One-shot and Few-shot Domain Adaptation

Domain adaptation of GANs is a problem of fine-tuning GAN models pretrained on a large dataset (e.g. StyleGAN) to a specific domain with few samples (e.g. painting faces, sketches, etc.). While there are many methods that tackle this problem in different ways, there are still many important questions that remain unanswered. In this paper, we provide a systematic and in-depth analysis of the domain adaptation problem of GANs, focusing on the StyleGAN model. We perform a detailed exploration of the most important parts of StyleGAN that are responsible for adapting the generator to a new domain depending on the similarity between the source and target domains. As a result of this study, we propose new efficient and lightweight parameterizations of StyleGAN for domain adaptation. Particularly, we show that there exist directions in StyleSpace (StyleDomain directions) that are sufficient for adapting to similar domains. For dissimilar domains, we propose Affine+ and AffineLight+ parameterizations that allows us to outperform existing baselines in few-shot adaptation while having significantly less training parameters. Finally, we examine StyleDomain directions and discover their many surprising properties that we apply for domain mixing and cross-domain image morphing. Source code can be found at https://github.com/AIRI-Institute/StyleDomain.

==> s1_intro_old.tex <==

\section{Introduction}
\label{sec:intro}
Recent years GANs \cite{goodfellow2014generative, karras2019style, karras2020analyzing, karras2021alias, brock2018large} show impressive results in image synthesis and offer many kinds of control over generated data. In particular, the state-of-the-art StyleGAN models \cite{karras2019style, karras2020analyzing, karras2021alias} allow a great number of semantic image manipulations by identifying corresponding directions in different latent spaces ($\mathcal{W}$, $\mathcal{W}+$, or StyleSpace). Between these three latent spaces the StyleSpace provides the most disentangled and interpretable controls for image editing. Such properties of StyleGAN models lead to many practical applications as image enhancement, editing, image-to-image translation, etc. 
%Especially style-based generators demonstrates highly semantically rich latent spaces. It allows to control many semantic attributes, in particular StyleSpace show good disentanglement. 
However, it comes at a price as the training of StyleGAN requires large high-quality dataset that significantly limits its applicability because there are many domains of data that are represented by only few images. 
%However, to get access to such abilities we need large high-quality dataset to train GAN for a target domain. The standard approach to deal with this problem is transfer learning. 

Transfer Learning (TL) is a standard approach to deal with the problem of training GANs with limited data. 
%The idea is to fine-tune the model pretrained on large dataset to a target domain with few samples. 
%StyleAlign introduces the term \emph{aligned models} for the case when we fine-tune the same architecture. The source pretrained model is called \emph{parent} and the obtained one is called \emph{child}. 
In the case of StyleGAN we fine-tune the model pretrained on the source domain $A$ to the target domain $B$.
There are many domain adaptation methods that tackle this problem in different ways depending on the distance between source $A$ and target $B$ domains. Some approaches consider the case when we adapt the StyleGAN to a far domain (e.g. faces $\rightarrow$ cars) and they typically fine-tune all its weights. Other methods deal with the target domains that are similar to the source one. For this case there are works that significantly reduce the parameter space for fine-tuning StyleGAN. However, all these papers focus on a specific aspect of the domain adaptation problem of StyleGAN and do not explore it in a more systematic way except the StyleAlign paper.

StyleAlign is the first attempt to perform in-depth analysis on the transfer learning of StyleGAN. They introduce the term of \emph{aligned models} as the models with the same architecture and one of them (the \emph{child}) is fine-tuned from the other (the \emph{parent}) to a new domain. They focus on aligned StyleGAN models and examine its properties. 
%The first important finding of this work is that the synthesis convolutional network of StyleGAN is mostly changed during domain adaptation. The second discovery is that the child model's latent spaces inherit rich semantics from the parent. 
While this work provides insightful analysis, some of its conclusions are incomplete or even misleading. For example, they find out that the synthesis convolutional network of StyleGAN is mostly changed during domain adaptation. From this observation one can conclude that this part is the most responsible for the transfer learning, however we show that it is not correct in most cases. It encourages us to revisit this analysis and perform more careful and thorough investigation. 
%Moreover, many other important questions about aligned StyleGAN models remain unanswered. 

In this work, we aim to provide the systematic and comprehensive analysis on the domain adaptation problem of StyleGAN models and tackle the most important questions that still remain unanswered. 
For example, what are main parts of StyleGAN mostly responsible for the tranfer learning to a new domain? How does it depend on the distance between the child and parent domains? Can we adapt the StyleGAN by finding some directions in its latent spaces or do we need necessarily fine-tune its synthesis convolutional network? Can we combine the results of domain adaptations to different domains in one StyleGAN model? 

Our investigation of the properties of the aligned StyleGAN models consists of several parts. First, in \Cref{sec:importance}, we identify what parts of the StyleGAN are responsible for its adaptation depending on the similarity between source and target domains. We discover that fine-tuning of the synthesis convolutional network is not always necessary and in some cases the affine layers can be sufficient for the transfer learning (see Figures). It suggests us to investigate the StyleSpace to utilize it for the domain adaptation. So, in the second part of our analysis, in \Cref{sec:styledirections}, we explore directions in the StyleSpace that can adapt StyleGAN to other domains. We first show that such directions exist (and we call it as \emph{StyleDomain directions}) and for similar target domains they demonstrate the comparable domain adaptation quality as the fine-tuning all weights of StyleGAN. Further we examine these StyleDomain directions and discover its surprising properties. For example, we show that we can sum up these directions to obtain new mixed domain, and they can be successfully applied to other aligned StyleGAN model. Overall, our findings contributes to a better understanding of the properties of aligned StyleGAN models. 

%There are many domain adaptation methods for GANs. Each of them tackle specific aspects (applications) of this problem. However, they do not explore what main parts of StyleGAN are mostly responsible for the tranfer learning to a new domain. There is single work StyleAlign that try to investigate this question and provide insightful analysis. They find out that the most important part is the synthesis convolutional network of StyleGAN. However,  it is not the whole truth because of the misleading experiment.  


%Tranfer learning for GANs. It is important for training GANs with limited data. It can be used for image-to-image problems. 

%There many methods for domain adaptation of GANs. Each of them tackle specific aspects (applications) of this problem. There is only one good work StyleAlign that analyzes deeply the problem of StyleGAN domain adaptation. They propose the term of aligned StyleGAN models. It is a first good attempt to comprehensively investigate this problem. 

%We conduct more reasonable experiments. We provide the comprehensive analysis of the problem of domain adaptation of the StyleGAN model: 
%1) we identify what parts of the StyleGAN model are responsible (sufficient) for adapting the generator to a new domain depending on the distance between source and target domains; 2) we explore the StyleSpace of StyleGAN and first show that there are directions in this space that can adapt the whole generator to new domains; 3) we examine these StyleSpace directions that correspond to different domains and discover their surprising properties: a) we can combine these directions to obtain new mixed domain, b) they can be successfully applied to other aligned StyleGAN model; our findings contributes to a better understanding of the observations from the StyleAlign paper (why aligned models are semantically aligned). 

Additionally, in \Cref{sec:practical}, we consider practical imrovements and applications that can be delivered by our analysis and findings. First, we significantly reduce and simplify the parameter space of the domain adaptation of StyleGAN and show that achieves the same quality as fine-tuning all its weights. Second, we examine different applications of StyleDomain directions such mixed domains and transfering adaptation between aligned StyleGAN models. Finally, we apply our findings to standard image-to-image translation and cross-domain morphing tasks and show that they can be easily solved in our framework. 

To summarize, we conduct a comprehensive empirical study on the StyleGAN domain adaptation problem and reveal its many interesting aspects. We first show that StyleSpace has rich semantics not only for image editing but also for domain adaptation. We leverage our findings for a variety of computer vision applications. 

%Our analysis and insights deliver many practical improvements and applications:
%1) we show that the training space for domain adaptation can be significantly reduced; 2) we can easily mix different domains by combining corresponding StyleSpace directions; 3) we can transfer face-specific styles to non-face domains (cats/dogs, churches, etc.); 4) we can easily combine semantic editing and domain adaptation (improve?); 5) we can easily solve I2I and transfer learning tasks; 6) we can easily morph between different domains. 
